Fine-Tuning Pretrained Language Models: Weight Initializations, Data Orders, and Early Stopping

Fine-tuning pretrained contextual word embedding models to supervised downstream tasks has become commonplace in natural language processing. This process, however, is often brittle: even with the same hyperparameter values, distinct random seeds can lead to substantially different results. To better understand this phenomenon, we experiment with four datasets from the GLUE benchmark, fine-tuning BERT hundreds of times on each while varying only the random seeds. We find substantial performance increases compared to previously reported results, and we quantify how the performance of the best-found model varies as a function of the number of fine-tuning trials. Further, we examine two factors influenced by the choice of random seed: weight initialization and training data order. We find that both contribute comparably to the variance of out-of-sample performance, and that some weight initializations perform well across all tasks explored. On small datasets, we observe that many fine-tuning trials diverge part of the way through training, and we offer best practices for practitioners to stop training less promising runs early. We publicly release all of our experimental data, including training and validation scores for 2,100 trials, to encourage further analysis of training dynamics during fine-tuning.

==> text/99_early_stopping_by_seed.tex <==
\subsection{Early stopping by seed}

Here we expand on the algorithm from Section \ref{sec:independent_es} and explore an early stopping algorithm that independently stops trials with least promising WI and DO seeds. We further examine in which conditions this can be advantageous.
% Estimating the performance of a WI or DO from a single experiment is too noisy, and in this section we explore an early stopping algorithm which utilizes multiple runs for a single seed to get a better estimate of performance.

Similarly to the algorithm described in Section \ref{sec:independent_es}, we start multiple runs for each seed. The main difference is that, when it is time to early stop, instead of stopping the least promising overall trials, we stop the ones with the worst WI and worst DO seeds.
A more complete description of this algorithm can be found in the appendix. \jdcomment{We should add this algorithm to the appendix.}

\paragraph{When early stopping by seed is helpful}
To better understand how WIs and DOs impact performance, we explore when early stopping by seeds is helpful. For comparison, we use a baseline which starts and stops the same number of experiments after training on the same fraction of the training budget. On the baseline, experiments are stopped based on individual performance, whereas in this algorithm, experiments for a given seed are all stopped based on the average performance for that seed.

Stopping a set of experiments with the same WI outperforms the independent baseline when the training budget before early stopping is small \jdcomment{some summary numbers here}. This is true across all datasets, and across varying computational budgets and. 
On SST, stopping a set of experiments with the same DO outperforms the baseline when early stopping about halfway through the full training budget, though on the three smaller datasets we see larger improvements when early stopping near the beginning of training. In all these scenarios, we observe small but consistent gains from stopping by seed  \jdcomment{some summary numbers here}.

\nascomment{if you present two algorithms, you have to take the same amount of care in explaining and evaluating each.  this subsection about the second algorithm needs to be either deleted (along with all references to it) or brought up to the same level of detail as 6.1}

==> text/99_old_early_stopping.tex <==


% \begin{itemize}
%     % \item In this section we examine an early stopping algorithm which allows for a practitioner to set up a set of experiments that meet a fixed budget.
%     \item Early stopping of individual experiments is fairly common. Often practitioners use an early stopping criteria like "stop once the best evaluation on validation data was more than X evaluations ago" or "the average loss over the last Y is not lower than the average of the Y before that". These have some hparams, and are mainly useful for detecting convergence or when a model has diverged, and future work can use our released data (like the loss at every weight update) to find the best way to do this kind of early stopping.
%     \item There are many ways to detect divergence during training, including early stopping of individual experiments (as described above), but our approach is useful even on larger datasets like SST where models don't typically diverge.
%     \item The fraction of models which diverge is interesting, though we find empirically it is different from the number of jobs we stop training early.
% \end{itemize}


% \subsection{Independent early stopping}
% \label{sec:independent_es}

%The most typical scenario when fine-tuning is not to have distinct random seeds controlling WI and DO. Here we examine a simple early stopping algorithm that does not take into account these factors separately, and is informed only by the validation performance of the models throughout training.





% \gamaga{I'd consider not including this as an algorithm, as it is fairly simple and can be described in words. Maybe we can do this if we include the more complex one.}
% \jdcomment{Okay then can you clean up the text description so it's as clear as an algorithm would be?}

% \begin{algorithm*}[tb]
%   \caption{Early Stopping}
%   \label{alg:early_stop}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} \# models $m$, \# initial steps $s_1$, \# additional steps $s_2$, \# models to keep $k$ 
%   \STATE models = getModelSamples($m$)
%   \STATE validationPerformances = trainAndEval(models, trainSteps=$s_1$)
%   \STATE modelsToKeep = getTopK(models, validationPerformances, $k$)
%   \STATE validationPerformances = trainAndEval(modelsToKeep, trainSteps=$s_2$)
%   \STATE \textbf{Return} getTopK(modelsToKeep, validationPerformances, 1)
% \end{algorithmic}
% \end{algorithm*}


% \nascomment{this doesn't go here, and the point as it's made now is too speculative}
% We expect more sophisticated algorithms that leverage early stopping such as Hyperband \cite{li2016hyperband} to yield even further improvements. \jdcomment{Can we say something here about how we tried Hyperband? @gabe do you have any details on those experiments?}\gamaga{yes, they are in our chat history. I could also re-run any particular experiment if you want. But per our previous discussions, not sure if we should include those}





% \begin{table}
% \setlength\tabcolsep{2.8pt}
%     \centering
%     \begin{tabular}{lcccc}
%                  & MRPC & RTE & CoLA & SST\\\hline
%     improvement (\%)& 0.47 & 0.98 & 0.41 & 0.05\\
%     std dev (\%)    & 0.36 & 0.28 & 0.17 & 0.02\\
%     \end{tabular}
%     \caption{The improvement provided by the early stopping algorithm presented in Section \ref{sec:independent_es}, averaged across different computational budgets.}
%     \label{tab:early_stop_improve}
% \end{table}

